An implementation of tensor product patch smoothers on GPU

We present a GPU implementation of vertex-patch smoothers for higher order finite element methods in two and three dimensions. Analysis shows that they are not memory bound with respect to GPU DRAM, but with respect to on-chip scratchpad memory. Multigrid operations are optimized through localization and reorganized local operations in on-chip memory, achieving minimal global data transfer and a conflict free memory access pattern. Performance tests demonstrate that the optimized kernel is at least 2 times faster than the straightforward implementation for the Poisson problem, across various polynomial degrees in 2D and 3D, achieving up to 36% of the peak performance in both single and double precision on Nvidia A100 GPU.

==> attic.tex <==
In this section, we test our algorithm with the model problem \eqref{eq:model} and let $f \equiv 1$. 
The resulting linear system is solved by the generalized minimal residual method (GMRES) preconditioned by a V-cycle with one pre- and post smoothing step. A relative residual reduction of $\delta = 10^{-9}$ uses as the stopping criterion. The fractional iterations according to Witte \cite{witte2021fast} is
\begin{equation*}
    n_{\mathrm{frac}}=n-1+\frac{\log \left(e_{n-1} / \varepsilon_{\mathrm{tol}}\right)}{\log \left(e_{n-1} / e_n\right)},
\end{equation*}
where $ \varepsilon_{tol} = e_0\delta$ and $e_n$ is the energy norm of the error and the Euclidean norm of the residual after $n$ steps of the GMRES algorithm. Note that multiplicative vertex patch smoother is effective considering that they only need three iterations or less for high order polynomial degrees, thus we consider fractional iterations for a more accurate measure of their convergence speed.

Experiments are presented in Table \ref{tab:GMRES_v_2d} and Table \ref{tab:GMRES_v_3d}. For each polynomial degree, the problem sizes are between $10^6$ and $10^9$ degrees of freedom in two dimensions, and between $10^6$ and $10^9$ in three dimensions on mesh level $L$.
As we can see, the number of steps is independent of the reﬁnement level in both cases. Furthermore, numerical results show that the number of steps required for convergence decreases with increasing of polynomial degree, indicating that vertex patch smoother is more suitable for higher order degrees.

\begin{table}[tp]
    \centering
    \caption{Fractional iterations $n_{\mathrm{frac}}$ for preconditioned GMRES method in two dimensions.}
    \label{tab:GMRES_v_2d}
    \renewcommand{\arraystretch}{1.5}
    \begin{tabular}{C{0.5cm}|C{0.7cm}C{0.7cm}C{0.7cm}C{0.7cm}
    C{0.7cm}C{0.7cm}C{0.7cm}C{0.7cm}C{0.7cm}C{0.7cm}}
        \hline
         \textbf{$L$} & $\mathbb{Q}_1$ & $\mathbb{Q}_2$ & $\mathbb{Q}_3$ &
         $\mathbb{Q}_4$ & $\mathbb{Q}_5$ & $\mathbb{Q}_6$ & $\mathbb{Q}_7$ &
         $\mathbb{Q}_8$ & $\mathbb{Q}_9$ & $\mathbb{Q}_{10}$ \\
        \hline
         3 & 2.8 & 2.9 & 2.4 & 2.1 & 2.0 & 1.9 & 1.8 & 1.8 & 1.7 & 1.7 \\
         4 & 5.0 & 3.5 & 2.9 & 2.4 & 2.3 & 2.2 & 2.1 & 1.9 & 1.9 & 1.9 \\
         5 & 5.5 & 4.1 & 2.9 & 2.7 & 2.4 & 2.3 & 2.1 & 2.0 & 1.9 & 1.9 \\
         6 & 5.8 & 4.2 & 2.8 & 2.7 & 2.4 & 2.3 & 2.1 & 2.0 & 1.9 & 1.8 \\
         7 & 5.8 & 4.2 & 2.7 & 2.6 & 2.3 & 2.2 & 2.0 & 2.0 & 1.8 & 1.8 \\
         8 & 5.7 & 4.0 & 2.6 & 2.5 & 2.3 & 2.2 & 2.0 & 1.9 & 1.8 & 1.8 \\
         9 & 5.4 & 3.8 & 2.5 & 2.5 & 2.2 & 2.2 & 2.0 & 1.9 & 1.8 & 1.8 \\
         10 & 5.2 & 3.7 & 2.5 & 2.5 & 2.2 & 2.2 & 2.0 & 1.9 & 1.8 & 1.8 \\
         11 & 4.8 & 3.7 & 2.5 & 2.5 & 2.2 & 2.2 & 2.0 & 1.9 & 1.8 & 1.8 \\
         12 & 4.7 & 3.7 & 2.5 & 2.5 & 2.2 & 2.2 & 2.0 & 1.9 & 1.8 & 1.8\\
        \hline
    \end{tabular}
\end{table}

\begin{table}[tp]
    \centering
    \caption{Fractional iterations $n_{\mathrm{frac}}$ for preconditioned GMRES method in three dimensions.}
    \label{tab:GMRES_v_3d}
    \renewcommand{\arraystretch}{1.5}
    \begin{tabular}{C{0.5cm}|C{0.7cm}C{0.7cm}C{0.7cm}C{0.7cm}
    C{0.7cm}C{0.7cm}C{0.7cm}C{0.7cm}}
        \hline
         \textbf{$L$} & $\mathbb{Q}_1$ & $\mathbb{Q}_2$ & $\mathbb{Q}_3$ &
         $\mathbb{Q}_4$ & $\mathbb{Q}_5$ & $\mathbb{Q}_6$ & $\mathbb{Q}_7$ &
         $\mathbb{Q}_8$ \\
         \hline
         3  &  3.8  &  3.2 &  2.9  & 2.6  & 2.4  & 2.2 & 2.0 & 2.0 \\
         4  &  4.2  &  3.8 &  3.1  & 2.7  & 2.5  & 2.3 & 2.1 & 2.0   \\
         5  &  4.7  &  3.9 &  3.0  & 2.7  & 2.5  & 2.3 & 2.1 & 2.0   \\
         6  &  4.7  &  3.9 &  2.9  & 2.6  & 2.4  & 2.3 & 2.1 & 2.0   \\
         7  &  4.6  &  3.7 &  2.8  & 2.5  & 2.4  & 2.2 & 2.1 & 1.9   \\
         8  &  4.5  &  3.6 &  2.8  & 2.5  & 2.3  & 2.0 & 2.0 & -  \\
        \hline
    \end{tabular}
\end{table}

\begin{table}[tp]
    \centering
    \caption{Comparison of vertex patch smoother and point Gauss–Seidel smoother for higher order elements in three dimensions. (iteration steps $n$ for preconditioned GMRES)}
    \label{tab:vp_GS_GMRES}
    \renewcommand{\arraystretch}{1.5}
    \begin{tabular}{lC{0.7cm}C{0.7cm}C{0.7cm}C{0.7cm}C{0.7cm}C{0.7cm}C{0.7cm}C{0.7cm}}
        \hline
           & $\mathbb{Q}_1$ & $\mathbb{Q}_2$ & $\mathbb{Q}_3$ &
         $\mathbb{Q}_4$ & $\mathbb{Q}_5$ & $\mathbb{Q}_6$ & $\mathbb{Q}_7$ &
         $\mathbb{Q}_8$ \\
         \hline
         point GS & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 \\
         vertex patch & 6 & 5 & 3 & 3 & 3 & 3 & 2 & 2 \\
        \hline
    \end{tabular}
\end{table}

\begin{table}[tp]
    \centering
    \caption{Arithmetic Throughput and Memory Throughput for {\it Fused CF} kernel in 3D.}
    \label{tab:perf_all}
    \renewcommand{\arraystretch}{1.5}
    \begin{tabular}{lcccc}
    \hline
     & \multicolumn{2}{c}{TFLOP/s (\% of peak)} & \multicolumn{2}{c}{Gbyte/s (\% of peak)} \\ 
    Degree & FP32 & FP64 & FP32 & FP64 \\
    \hline 
    1 &  2.371 (13.3\%) & 1.412 (16.0\%)  & 145.88 (7.15\%) & 169.64 (8.32\%)\\
    2 &  2.823 (15.9\%) & 1.838 (20.9\%)  & 178.15 (8.74\%) &  235.08 (11.52\%) \\ 
    3 &  4.282 (24.2\%) & 2.429 (27.6\%)  & 253.04 (12.41\%) &  286.13 (14.03\%) \\
    4 &  5.299 (29.9\%) & 2.848 (32.3\%) & 238.57 (11.70\%) & 272.09 (13.35\%) \\
    5 &  6.336 (35.8\%) & 3.258 (37.0\%)  & 255.95 (12.57\%) & 260.47 (12.79\%) \\
    6 &  6.316 (35.7\%) & 3.310 (37.6\%)  & 218.90 (10.75\%) &  226.91 (11.14\%) \\
    7 &  6.382 (36.1\%) & 3.191 (36.3\%)  & 192.92 (9.48\%) & 191.03 (9.37\%) \\
    8 &  5.281 (29.8\%) & 2.537 (28.8\%)  & 140.86 (6.91\%) & 112.30 (5.51\%) \\
    \hline
    \end{tabular}
\end{table}


\begin{table}[tp]
    \centering
    \caption{The profiler report of {\it Fused} kernel in 3D}
    \label{tab:profile_kernel_3d}
    \renewcommand{\arraystretch}{1.5}
    \begin{tabular}{c|ccccccccc}
        \hline
        $p$ & \# T & \# Regs & Shmem & \# TB & TFLOP & Occu. & L1 & L2 & Allocatable TB\\
        \hline 
        2 & 50 & 32 & 4.20 & 32 & 2.371 & 97.32 & 96.37 & 17.87 & 32/32/32\\
        3 & 49 & 32 & 5.88 & 24 & 2.832 & 73.39 & 95.27 & 27.94 & 32/32/24 \\ 
        4 & 81 & 48 & 12.31 & 12 & 4.282 & 55.27 & 96.73 & 25.16 & 21/13/12 \\
        5 & 121 & 56 & 22.26 & 7 & 5.299 & 43.16 & 96.37 & 24.22 & 16/9/7\\
        6 & 169 & 56 & 36.50 & 4 & 6.336 & 37.01 & 91.58 & 19.52 & 10/6/4 \\
        7 & 225 & 64 & 55.80 & 2 & 6.382 & 24.69 & 90.49 & 17.13 & 8/4/2 \\
        % 8 & 289 & 64 & 80.92 & 2 & 5.281 & 31.02 & 84.08 & 11.98 & 6/3/2 \\
        \hline
        \multicolumn{9}{l}{\small  \# T: Threads per block, \# Regs: Registers per threads.} \\
        \multicolumn{9}{l}{\small Shmem: Dynamic shared memory per block [Kbyte/block].} \\
        \multicolumn{9}{l}{\small \# TB: Thread blocks per multiprocessor.} \\
        \multicolumn{9}{l}{\small Occu.: Achieved occupancy of each multiprocessor[\%].} \\ 
        \multicolumn{9}{l}{\small L1, L2: L1/TEX cache, L2 cache Throughput [\%].} \\
        \multicolumn{10}{l}{\small Allocatable TB: Allocatable Blocks per SM based on \#T/\#Regs/Shmem.} \\
        \end{tabular}
\end{table}
